ManiFoundation Model for General-Purpose Robotic Manipulation of Contact Synthesis with Arbitrary Objects and Robots

To substantially enhance robot intelligence, there is a pressing need to develop a large model that enables general-purpose robots to proficiently undertake a broad spectrum of manipulation tasks, akin to the versatile task-planning ability exhibited by LLMs. The vast diversity in objects, robots, and manipulation tasks presents huge challenges. Our work introduces a comprehensive framework to develop a foundation model for general robotic manipulation that formalizes a manipulation task as contact synthesis. Specifically, our model takes as input object and robot manipulator point clouds, object physical attributes, target motions, and manipulation region masks. It outputs contact points on the object and associated contact forces or post-contact motions for robots to achieve the desired manipulation task. We perform extensive experiments both in the simulation and real-world settings, manipulating articulated rigid objects, rigid objects, and deformable objects that vary in dimensionality, ranging from one-dimensional objects like ropes to two-dimensional objects like cloth and extending to three-dimensional objects such as plasticine. Our model achieves average success rates of around 90\%. Supplementary materials and videos are available on our project website at https://manifoundationmodel.github.io/.

==> tex/ack.tex <==
\input{root_supp}
\input{}

==> tex/llm.tex <==
% In the complex task of generating trajectories for floating objects based on free-form language instructions, a comprehensive approach that integrates strong contextual understanding and multimodal reasoning is essential. 
Generating collision-free dense trajectories for floating objects and portions of deformable objects is not easy. 
The reason is that the planner should know 
To address these challenges, our planner incorporates three key components: A sparse trajectory planner based on large language models~\cite{achiam2023gpt}, an object detection model~\cite{ren2024grounded}, and a rapidly-exploring random Tree (rrt)-connect motion planner~\cite{844730}.

In the real world, the robot captures the surrounding environment using the camera mounted on its head, producing an RGB-D image, $o_{t}$, to estimate the position and orientation of each object within $o_{t}$. 
We employ Grounded-SAM~\cite{ren2024grounded} to generate 2D bounding boxes around each object, using object names as prompts. 
These 2D coordinates are then projected onto 3D space, $s_{i}$, corresponding to the robot's perspective coordinates.

We reconstruct 3D point clouds and meshes for each object using Gaussian splatting and position them in the Jade simulator according to their 3D coordinates, $s_{i}$ effectively simulating the real-world environment.

The LLM serves as our primary world model, offering a universal understanding of the concepts essential for task planning and constraint adherence. In our task, the LLM identifies the starting points for planning (e.g., the initial position of the apple), areas to avoid for collision prevention (e.g., the vessel), and the target location (e.g., the interior of the microwave). 
It then generates a series of sparse pose changes, indicating the basic coordinates to which the object should be moved. 
However, trajectories proposed by the LLM are not entirely reliable, as the model is not provided with comprehensive physical details of the environment, such as the precise dimensions of the microwave’s interior. Relying solely on linear interpolation of key waypoints could, therefore, result in potential collisions with the environment.

we employ a sampling-based motion planning technique, RRT-connect~\cite{844730}, which is enhanced with collision awareness based on the distance between point clouds. 
This method allows us to refine the trajectory into a dense, collision-avoidant path, ensuring safe and effective navigation within the simulated environment.


==> tex/prob.tex <==
In this work, we choose to represent objects with point clouds. Here, objects can be articulated rigid objects, rigid objects, 1D deformable objects~(such as rope), 2D deformable objects~(such as cloth, paper, or plastic bags), 3D deformable objects~(elastoplastic objects, plasticine). Our framework assumes an object manipulation task can be represented by a sequence of object point clouds~(subgoals).

Given the object trajectory, this work aims to develop a foundation model $\mathcal{F}$ that takes as input 1) the object's current point cloud to represent the object shape, 3) the object target point cloud or the object current point cloud point-wise target motion to represent the manipulation task description, 2) physical attributes (such as friction coefficients, Young’s modulus, etc) to reflect the object types,  3) robot descriptions such as the URDF, 4) manipulation region masks if needed, for example, the task requires the robot to grasp the pan's handle. The foundation model $\mathcal{F}$ outputs the contact points, contact force, or post-contact motion, so that robots can manipulate the object toward its target state.

For how to translate a manipulation task description into a feasible object trajectory, our pipeline leverages the LLMs/LVMs to generate waypoints of the rigid body 6D poses or leverage the goal RGBD image of the deformable objects' target state.
